Khuri-Treiman equations for $3\pi$ decays of particles with spin

Khuri-Treiman equations have proven to be a useful theoretical tool in the analysis of 3-body decays, specially into the $3\pi$ final state. In this work we present in full detail the necessary generalization of the formalism to study the decays of particles with arbitrary spin, parity, and charge conjugation. To this extent, we find it most convenient to work with helicity amplitudes instead of the so-called invariant amplitudes, specially when dealing with the unitarity relations. The isobar expansions in the three possible ($s$-, $t$-, and $u$-) final channels are related with the appropriate crossing matrices. We pay special attention to the kinematical singularities and constraints of the helicity amplitudes, showing that these can be derived by means of the crossing matrix.

==> figures/tminmax_A.tex <==
\nextgroupplot[anchor=north west,
%at={($(lplots c1r1.north east) + (1.50cm,-1.50cm)$)},
%at={(7cm,5cm)},
scale=1.5,
ticks=none,
xmin=-4*\m^2,xmax=tmax(\sejA)+8*\m^2,
ymin=-0.4*\yymax,
ymax=+0.4*\yymax,
height=3cm,
title style={at={(0.50,0.95)}},
title=$\displaystyle 4m^2 \leqslant s \leqslant \frac{M^2-m^2}{2}$,
]

\addplot[PathStyle,->-] coordinates{({tmin(\sejA)},{+\eps}) ({tmax(\sejA)},{+\eps})};
\addplot[cut]      coordinates{({4*\m^2},{0.0}) ({tmax(\sejA)+8*\m^2},{0.0})} ;

\node[color=Black,draw,fill=Black,circle,minimum size=3pt,inner sep=2pt,label=above:{$4m^2$}] at ({4*\m^2},0) {};
\node[color=Path,draw,fill=Path,circle,minimum size=3pt,inner sep=2pt,label=above:{$\textcolor{Path}{t_-(s)}$}] at ({tmin(\sejA)},{+\eps}) {};
\node[color=Path,draw,fill=Path,circle,minimum size=3pt,inner sep=2pt,label=above:{$\textcolor{Path}{t_+(s)}$}] at ({tmax(\sejA)},{+\eps}) {};




==> figures/tminmax_B.tex <==
\nextgroupplot[scale=1.5,
ticks=none,
xmin=-6*\m^2,xmax=tmax(\sejB)+6*\m^2,
ymin=-0.4*\yymax,
ymax=+0.4*\yymax,
height=3cm,
title style={at={(0.5,0.95)}},
title=$\displaystyle \frac{M^2-m^2}{2} \leqslant s \leqslant s_-$
]

\addplot[cut]      coordinates{({4*\m^2},{0.0}) ({tmax(\sejB)+16*\m^2},{0.0})} ;
\draw[PathStyle,->-] ({tmin(\sejB)},{-\eps}) -- (3.25*\m^2,{-\eps});
\draw[PathStyle,->-] (3.25*\m^2,{-\eps}) -- (3.25*\m^2,{+\eps});
\draw[PathStyle,->-] (3.25*\m^2,{+\eps}) -- ({tmax(\sejB)},{+\eps});

\node[color=Black,draw,fill=Black,circle,minimum size=3pt,inner sep=2pt,label=left:{$4m^2$}] at ({4*\m^2},0) {};
\node[color=Path,draw,fill=Path,circle,minimum size=3pt,inner sep=2pt,label=below:{$\textcolor{Path}{t_-(s)}$}] at ({tmin(\sejB)},{-\eps}) {};
\node[color=Path,draw,fill=Path,circle,minimum size=3pt,inner sep=2pt,label=above:{$\textcolor{Path}{t_+(s)}$}] at ({tmax(\sejB)},{+\eps}) {};


==> figures/tminmax_C.tex <==
\nextgroupplot[scale=1.5,
ticks=none,
xmin=3*\m^2,xmax=trea(\sejC)+1*\m^2,
ymin=-\yymax,ymax=\yymax,
height=4.5cm,
title style={at={(0.50,0.95)}},
title=$\displaystyle s_- \leqslant s \leqslant M^2-5m^2$
]

\addplot[cut]      coordinates{({4*\m^2},{0.0}) ({trea(\sejC)+16*\m^2},{0.0})} ;
\draw[PathStyle,->-] ({trea(\sejC)},{-tima(\sejC)}) -- ({trea(\sejC)},{-\eps});
\draw[PathStyle,->-] ({trea(\sejC)},{-\eps}) -- (3.9*\m^2,{-\eps});
\draw[PathStyle,->-] (3.9*\m^2,{-\eps}) -- (3.9*\m^2,{+\eps});
\draw[PathStyle,->-] (3.9*\m^2,{+\eps}) -- ({trea(\sejC)},{+\eps});
\draw[PathStyle,->-] ({trea(\sejC)},{+\eps}) -- ({trea(\sejC)},{tima(\sejC)});

\node[color=Black,draw,fill=Black,circle,minimum size=3pt,inner sep=2pt,label=left:{$4m^2$}] at ({4*\m^2},0) {};
\node[color=Path,draw,fill=Path,circle,minimum size=3pt,inner sep=2pt,label=below:{$\textcolor{Path}{t_-(s)}$}] at ({trea(\sejC)},{-tima(\sejC)}) {};
\node[color=Path,draw,fill=Path,circle,minimum size=3pt,inner sep=2pt,label=above:{$\textcolor{Path}{t_+(s)}$}] at ({trea(\sejC)},{+tima(\sejC)}) {};




==> figures/tminmax_D.tex <==
\nextgroupplot[scale=1.5,
ticks=none,
xmin=trea(\sejD)-2*\m^2,xmax=8*\m^2,
ymin=-\yymax,ymax=\yymax,
height=4.5cm,
title style={at={(0.50,0.95)}},
title=$\displaystyle M^2-5m^2 \leqslant s \leqslant s_+$]
]

\addplot[cut]      coordinates{({4*\m^2},{0.0}) ({trea(\sejD)+16*\m^2},{0.0})} ;
%\draw[PathStyle,->-] ({trea(\sejC)},{-tima(\sejC)}) -- ({trea(\sejC)},{-\eps});
%\draw[PathStyle,->-] ({trea(\sejC)},{-\eps}) -- (3.5*\m^2,{-\eps});
%\draw[PathStyle,->-] (3.5*\m^2,{-\eps}) -- (3.5*\m^2,{+\eps});
%\draw[PathStyle,->-] (3.5*\m^2,{+\eps}) -- ({trea(\sejC)},{+\eps});
%\draw[PathStyle,->-] ({trea(\sejC)},{+\eps}) -- ({trea(\sejC)},{tima(\sejC)});

\draw[PathStyle,->-] ({trea(\sejD)},{-tima(\sejD)}) -- ({trea(\sejD)},{+tima(\sejD)});

\node[color=Black,draw,fill=Black,circle,minimum size=3pt,inner sep=2pt,label=below:{$4m^2$}] at ({4*\m^2},0) {};
\node[color=Path,draw,fill=Path,circle,minimum size=3pt,inner sep=2pt,label=below:{$\textcolor{Path}{t_-(s)}$}] at ({trea(\sejD)},{-tima(\sejD)}) {};
\node[color=Path,draw,fill=Path,circle,minimum size=3pt,inner sep=2pt,label=above:{$\textcolor{Path}{t_+(s)}$}] at ({trea(\sejD)},{+tima(\sejD)}) {};



==> figures/tminmax_E.tex <==
\nextgroupplot[scale=1.5,
  at = { ($ ( $ (rplots c1r2.south west) + (0,-100pt)$ )!0.5!(rplots c2r2.south east) $ ) },
ticks=none,
xmin=tmin(\sejE)-4*\m^2,xmax=16*\m^2,
ymin=-\yymax,ymax=\yymax,
height=3.5cm,
title style={at={(0.50,0.95)}},
title=$\displaystyle s_+ \leqslant s$
]

\addplot[cut]      coordinates{({4*\m^2},{0.0}) ({16*\m^2},{0.0})} ;
\draw[PathStyle,->-] ({tmin(\sejE)},{0.00}) -- ({tmax(\sejE)},{0.00});

\node[color=Black,draw,fill=Black,circle,minimum size=3pt,inner sep=2pt,label=above:{$4m^2$}] at ({4*\m^2},0) {};
\node[color=Path,draw,fill=Path,circle,minimum size=3pt,inner sep=2pt,label=above:{$\textcolor{Path}{t_-(s)}$}] at ({tmin(\sejE)},{0.00}) {};
\node[color=Path,draw,fill=Path,circle,minimum size=3pt,inner sep=2pt,label=above:{$\textcolor{Path}{t_+(s)}$}] at ({tmax(\sejE)},{0.00}) {};


==> figures/tminmax_cp.tex <==
\nextgroupplot[scale=2,
    ticks=none,
  xmin=-12*\m^2,
  xmax=+15*\m^2,
%  ymax=(\mA-\m)^2+4*\m^2,
%  ymin=tmin((\mA+\m)^2+16*\m^2),
]

\addplot[domain=4*\m^2:\m*(\mA+\m),samples=30,variable=\s,tmin,->-] ({tmin(\s)},{+1*\epsB});
\addplot[domain=4*\m^2:\m*(\mA+\m),samples=30,variable=\s,tmax,->-] ({tmax(\s)},{+2*\epsB});

\addplot[domain=\m*(\mA+\m):(\mA^2-\m^2)/2,samples=60,variable=\s,tmin,->-] ({tmin(\s)},{+1*\epsB});
\addplot[domain=\m*(\mA+\m):(\mA^2-\m^2)/2,samples=60,variable=\s,tmax,->-] ({tmax(\s)},{+2*\epsB});

\addplot[domain=(\mA^2-\m^2)/2:(\mA-\m)^2,samples=100,variable=\s,tmin,->-] ({tmin(\s)},{-1*\epsB});
\addplot[domain=(\mA^2-\m^2)/2:(\mA-\m)^2,samples=100,variable=\s,tmax,->-] ({tmax(\s)},{+2*\epsB});

\addplot[domain=(\mA-\m)^2:(\mA-\m)^2 + 0.25*\m^2,samples=60,variable=\s,tmin] ({trea(\s)},{-1*\epsB-tima(\s)});
\addplot[domain=(\mA-\m)^2:(\mA-\m)^2 + 0.25*\m^2,samples=60,variable=\s,tmax] ({trea(\s)},{+2*\epsB+tima(\s)});

\addplot[domain=(\mA-\m)^2 + 0.25*\m^2:\mA^2-5*\m^2,samples=30,variable=\s,tmin,->-] ({trea(\s)},{-1*\epsB-tima(\s)});
\addplot[domain=(\mA-\m)^2 + 0.25*\m^2:\mA^2-5*\m^2,samples=30,variable=\s,tmax,->-] ({trea(\s)},{+2*\epsB+tima(\s)});

\addplot[domain=\mA^2-5*\m^2:(\mA+\m)^2,samples=30,variable=\s,tmin,->-] ({trea(\s)},{-1*\epsB-tima(\s)});
\addplot[domain=\mA^2-5*\m^2:(\mA+\m)^2,samples=30,variable=\s,tmax,->-] ({trea(\s)},{+2*\epsB+tima(\s)});

\addplot[domain=(\mA+\m)^2:(\mA+\m)^2+1*\m^2,samples=30,variable=\s,tmin] ({tmin(\s)},{-1*\epsB});
\addplot[domain=(\mA+\m)^2:(\mA+\m)^2+1*\m^2,samples=30,variable=\s,tmax] ({tmax(\s)},{+2*\epsB});

\addplot[domain=(\mA+\m)^2+1*\m^2:(\mA+\m)^2+10*\m^2,samples=30,variable=\s,tmin,->-] ({tmin(\s)},{-1*\epsB});
\addplot[domain=(\mA+\m)^2+1*\m^2:(\mA+\m)^2+100*\m^2,samples=30,variable=\s,tmax,->-] ({tmax(\s)},{+2*\epsB});

\addplot[cut]      coordinates{({4.25*\m^2},{0.0}) ({100*\m^2},{0.0})} ;
\node[color=Black,draw,fill=Black,circle,minimum size=1pt,inner sep=1pt,label=left:{$4m^2$}] at ({4.25*\m^2},0) {};

%\node[color=ctmax,draw,fill=ctmax,circle,minimum size=1pt,inner sep=1pt,label=above:{$t_+(s_-)$} at ({trea((\mA-\m)^2)},{+2*\epsB}) {};
%\node[color=ctmax,draw,fill=ctmax,circle,minimum size=1pt,inner sep=1pt,label=above:{$t_+(s_-)$} at ({6*\m^2)},{0.02}) {};

\node[color=ctmax,draw,fill=ctmax,circle,minimum size=2pt,inner sep=2pt,label=above right:{\textcolor{ctmax}{$t_+(s_-)$}}] at ({trea((\mA-\m)^2)},{+2*\epsB}) {};
\node[color=ctmin,draw,fill=ctmin,circle,minimum size=2pt,inner sep=2pt,label=below right:{\textcolor{ctmin}{$t_-(s_-)$}}] at ({trea((\mA-\m)^2)},{-1*\epsB}) {};

\node[color=ctmax,draw,fill=ctmax,circle,minimum size=2pt,inner sep=2pt,label=above right:{\textcolor{ctmax}{$t_+(M^2-5m^2)$}}] at ({trea(\mA^2-5*\m^2)},{+2*\epsB+tima(\mA^2-5*\m^2)}) {};
\node[color=ctmin,draw,fill=ctmin,circle,minimum size=2pt,inner sep=2pt,label=below right:{\textcolor{ctmin}{$t_-(M^2-5m^2)$}}] at ({trea(\mA^2-5*\m^2)},{-1*\epsB-tima(\mA^2-5*\m^2)}) {};

\node[color=ctmax,draw,fill=ctmax,circle,minimum size=2pt,inner sep=2pt,label=above right:{\textcolor{ctmax}{$t_+(s_+)$}}] at ({trea((\mA+\m)^2)},{+2*\epsB}) {};
\node[color=ctmin,draw,fill=ctmin,circle,minimum size=2pt,inner sep=2pt,label=below left:{\textcolor{ctmin}{$t_-(s_+)$}}] at ({trea((\mA+\m)^2)},{-1*\epsB}) {};

\draw[tmin] (4*\m^2,\epsB) arc (90:270:\epsB);


==> figures/tminmax_tminmax.tex <==
\nextgroupplot[scale=2,
    ticks=none,
  xmin=3.8*\m^2,
  xmax=(\mA+\m)^2+4*\m^2,
  ymax=(\mA-\m)^2+2*\m^2,
  ymin=tmin((\mA+\m)^2+4*\m^2),
%title style={at={(0.50,0.95)}},
%title=$(a)$,
]

\addplot[samples=10,variable=\s,auli] ({\s},{4*\m^2});
\addplot[samples=10,variable=\s,auli] ({\s},{\m*(\mA+\m)});
\addplot[samples=10,variable=\s,auli] ({\s},{(\mA-\m)^2});

\addplot[samples=10,variable=\t,auli] ({4*\m^2},{\t});
\addplot[samples=10,variable=\t,auli] ({(\mA-\m)^2},{\t});
\addplot[samples=10,variable=\t,auli] ({\mA^2-5*\m^2},{\t});
\addplot[samples=10,variable=\t,auli] ({(\mA^2+\m^2)/2},{\t});
\addplot[samples=10,variable=\t,auli] ({(\mA+\m)^2},{\t});

\addplot[domain=4*\m^2:16*\m^2,samples=30,variable=\s,tmin] {tmin(\s)};
\addplot[domain=4*\m^2:16*\m^2,samples=30,variable=\s,tmax] {tmax(\s)};

\addplot[domain=16*\m^2:(\mA-\m)^2-4*\m^2,samples=30,variable=\s,tmin] {tmin(\s)};
\addplot[domain=16*\m^2:(\mA-\m)^2-4*\m^2,samples=30,variable=\s,tmax] {tmax(\s)};

\addplot[domain=(\mA-\m)^2-4*\m^2:(\mA-\m)^2,samples=30,variable=\s,tmin] {tmin(\s)};
\addplot[domain=(\mA-\m)^2-4*\m^2:(\mA-\m)^2,samples=30,variable=\s,tmax] {tmax(\s)};

\addplot[domain=(\mA-\m)^2:(\mA+\m)^2,samples=10,variable=\s,tmin] {-\epsC+trea(\s)};
\addplot[domain=(\mA-\m)^2:(\mA+\m)^2,samples=10,variable=\s,tmax] {+\epsC+trea(\s)};

\addplot[domain=(\mA+\m)^2:(\mA+\m)^2+\m^2,samples=50,variable=\s,tmin] {tmin(\s)};
\addplot[domain=(\mA+\m)^2:(\mA+\m)^2+\m^2,samples=50,variable=\s,tmax] {tmax(\s)};

\addplot[domain=(\mA+\m)^2+\m^2:(\mA+\m)^2+16*\m^2,samples=50,variable=\s,tmin] {tmin(\s)};
\addplot[domain=(\mA+\m)^2+\m^2:(\mA+\m)^2+16*\m^2,samples=50,variable=\s,tmax] {tmax(\s)};

\node[label={[rotate=0,anchor=north east]:{\textcolor{AuxLin}{$t=4m^2$}}}]   at ({\mA^2+12*\m^2},{4*\m^2     -0.25*\m^2}) {};
\node[label={[rotate=0,anchor=south east]:{\textcolor{AuxLin}{$t=m(M+m)$}}}] at ({\mA^2+12*\m^2},{\m*(\mA+\m)-1.00*\m^2}) {};
\node[label={[rotate=0,anchor=south east]:{\textcolor{AuxLin}{$t=s_-$}}}]    at ({\mA^2+12*\m^2},{(\mA-\m)^2 -3.50*\m^2}) {};

%\node[label={[rotate=90]above:{\textcolor{AuxLin}{$s=s_-$}}}]  at ({(\mA-\m)^2},{-8.5*\m^2}) {};
%\node[label={[rotate=90]above:{\textcolor{AuxLin}{$s=s_+$}}}]  at ({(\mA+\m)^2},{-8.5*\m^2}) {};
%\node[label={[rotate=90]below:{\textcolor{AuxLin}{$s=4m^2$}}}] at ({(2*\m)^2},{-7.5*\m^2}) {};
%\node[label={[rotate=90]above:{\textcolor{AuxLin}{$s=\frac{M^2-m^2}{2}$}}}] at ({(\mA^2-\m^2)/2},{-7*\m^2}) {};
%\node[label={[rotate=90]above:{\textcolor{AuxLin}{$s=M^2-5m^2$}}}] at ({\mA^2-5*\m^2},{-6*\m^2}) {};


\node[label={[rotate=90,anchor=south west]above:{\textcolor{AuxLin}{$s=s_-$}}}]               at ($({(\mA-\m)^2}      ,0) + (rel axis cs:0,-0.35)$) {};
\node[label={[rotate=90,anchor=south west]above:{\textcolor{AuxLin}{$s=s_+$}}}]               at ($({(\mA+\m)^2}      ,0) + (rel axis cs:0,-0.35)$) {};
\node[label={[rotate=90,anchor=south west]above:{\textcolor{AuxLin}{$s=\frac{M^2-m^2}{2}$}}}] at ($({(\mA^2-\m^2)/2}  ,0) + (rel axis cs:0,-0.35)$) {};
\node[label={[rotate=90,anchor=south west]above:{\textcolor{AuxLin}{$s=4m^2$}}}]              at ($(0.14              ,0) + (rel axis cs:0,-0.35)$) {};
\node[label={[rotate=90,anchor=south west]above:{\textcolor{AuxLin}{$s=M^2-5m^2$}}}]          at ($({\mA^2-5*\m^2}    ,0) + (rel axis cs:0,-0.35)$) {};

% \end{axis}

%\node[color=AuxLin,draw,fill=AuxLin,circle,minimum size=1pt,inner sep=1pt,label={[rotate=90]right:{$s_-$}] at ({(\mA-\m)^2},{-16*\m^2}) {};



==> preamble_stuff/TikZsettings.tex <==
\tikzset{>=stealth'}
\tikzset{->-/.style={decoration={
  markings,
  mark=at position .63 with {\arrow{>}}},postaction={decorate}}}
\tikzset{zigzag/.style={decorate, decoration=zigzag}}
\tikzset{bra/.style={Black,thick,densely dashed}}
\tikzset{pion/.style={color=Black,mark=none,very thick}}
\tikzset{aone/.style={draw=Black,very thick,double}}
\pgfplotsset{mdl/.style={ color=Gold1,mark=none,line width=0.5pt,dash pattern=on 2.2pt off 1.5pt}}
\pgfplotsset{mmdl/.style={color=DodgerBlue1,mark=none,line width=1.0pt}}
\pgfplotsset{bou/.style={color=Black,mark=none,line width=1.0pt}}

%\pgfmathsetmacro{\m}{0.139}
%\pgfmathsetmacro{\mA}{1.260}
%\pgfmathsetmacro{\Sigma}{\mA^2 + 3*\m^2}


%\tikzset{collision/.style={draw=Black,thick,fill=gray,star,star points=12,star point ratio=1.8,minimum size=15pt}}

\tikzset{collision/.style={circle,draw=Black,thick,fill=gray,minimum size=15pt}}

\tikzset{cross/.style={cross out, draw=black, minimum size=2*(#1-\pgflinewidth), inner sep=0pt, outer sep=0pt},
%default radius will be 1pt. 
cross/.default={1pt}}

==> preamble_stuff/shorthands.tex <==
\renewcommand{\arraystretch}{1.2}
\newcommand{\Braket}[3]{\left\langle #1\vphantom{#2}\vphantom{#3} \right\rvert #2\vphantom{#1}\vphantom{#3} \left\lvert #3\vphantom{#1}\vphantom{#2} \right\rangle}
\newcommand{\braket}[3]{\left\langle #1 \right\rvert #2 \left\lvert #3 \right\rangle}
\newcommand{\braketno}[2]{\left\langle \vphantom{#2} #1 \right\rvert  \left. \vphantom{#1} #2  \right\rangle}

\newcommand{\CG}[3]{\left\langle #1 ; #2 \vphantom{#3} \right\rvert\left.\!\vphantom{#1}\vphantom{#2}#3\right\rangle}

\newcommand{\daniel}[1]{{\bf \color{DarkOrchid} Daniel:  #1}\xspace}
\newcommand{\danielcor}[2]{{\color{DarkOrchid} Daniel:\st{#1}{\bf #2}}\xspace}

\newcommand{\lao}[1]{\lambda_{X}(#1)}
\newcommand{\lap}[1]{\lambda_{\pi}(#1)}
\newcommand{\sqa}[1]{\sqrt{\lao{#1}}}
\newcommand{\sqp}[1]{\sqrt{\lap{#1}}}
\newcommand{\sqs}{\sqrt{s}}
\newcommand{\sqt}{\sqrt{t}}

\newcommand{\Disc}{\text{Disc }}
\newcommand{\diag}{\text{diag}}
\newcommand{\nand}{\text{ and }}
\newcommand{\mand}{\quad \text{ and } \quad}

%$ Shorthands for H's
\newcommand{\Hlam}[2]{\mAhat^{(#1)}_{#2}} %H^{(s)}_\lambda
\newcommand{\Hhat}[2]{\hat{\mA}^{(#1)}_{#2}}
\renewcommand{\hbar}[2]{a^{(#1)}_{#2}}
\newcommand{\Hbar}[2]{\bar{\mA}^{(#1)}_{#2}}

%% Shorthands for primed quanties
\newcommand{\jmax}{{j_{\text{max}}}}
\newcommand{\lamp}{{\lambda^\prime}}
\newcommand{\jp}{{j^\prime}}
\newcommand{\Ip}{{I^\prime}}

\newcommand{\modk}{\lvert \vec{p}_X \rvert}

\newcommand{\Eq}[1]{Eq.~\eqref{#1}}
\newcommand{\Eqs}[1]{Eqs.~\eqref{#1}}

\newcommand\bsub{\begin{subequations}}
\newcommand\esub{\end{subequations}}


%\renewcommand{\mA}{\mathcal{A}}
\newcommand{\mA}{{\mathcal{A}}}
\newcommand{\mAhat}{\hat{\mathcal{A}}}
\newcommand{\Ahat}{\hat{A}}

%%%%%%%%%%% to define principal value integrals
\def\Xint#1{\mathchoice{\XXint\displaystyle\textstyle{#1}}%
{\XXint\textstyle\scriptstyle{#1}}%
{\XXint\scriptstyle\scriptscriptstyle{#1}}%
{\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
\!\int}
\def\XXint#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$}\vcenter{\hbox{$#2#3$}}\kern-.5\wd0}}
\def\ddashint{\Xint=}
\def\dashint{\Xint-}
\def\pvint{\Xint-}


\hyphenation{thresh-old}

